Unleashing the Power of Visual Prompting At the Pixel Level

This paper presents a simple and effective visual prompting method for adapting pre-trained models to downstream recognition tasks. Our method includes two key designs. First, rather than directly adding together the prompt and the image, we treat the prompt as an extra and independent learnable component. We show that the strategy of reconciling the prompt and the image matters, and find that warping the prompt around a properly shrinked image empirically works the best. Second, we re-introduce two "old tricks" commonly used in building transferable adversarial examples, i.e., input diversity and gradient normalization, into visual prompting. These techniques improve optimization and enable the prompt to generalize better. We provide extensive experimental results to demonstrate the effectiveness of our method. Using a CLIP model, our prompting method sets a new record of 82.8% average accuracy across 12 popular classification datasets, substantially surpassing the prior art by +5.6%. It is worth noting that this prompting performance already outperforms linear probing by +2.1% and can even match fully fine-tuning in certain datasets. In addition, our prompting method shows competitive performance across different data scales and against distribution shifts. The code is publicly available at https://github.com/UCSC-VLAA/EVP.

==> paragraphs/limitation.tex <==
\section{Limitation}

\textcolor{blue}{As shown in Section 4.1, our proposed EVP significantly outperforms the previous state-of-the-art visual prompting method, and is even stronger than linear probing. However, with non-clip models, our simple one-to-one matching strategy does not yet achieve competitive results to linear probing.
This motivates us that there is still plenty of room for improvement
(e.g., by exploring more sophisticated one-to-multiple or even multiple-to-multiple matching strategies) in the future.}



